Solving Large-Scale Two-Echelon Location Routing Problems in City Logistics

Logistic service providers increasingly focus on two-echelon distribution systems to efficiently manage thousands of deliveries in urban environments. Effectively operating such systems requires designing cost-efficient delivery networks while addressing the challenges of increasing e-commerce demands. In this context, we focus on a two-echelon location routing problem with mobile depots and direct shipment, where decisions involve locating micro-depots, and designing first and second-level routes. Our model also incorporates the flexibility of direct shipments from the main depot to customers. To solve such large-scale problems efficiently, we propose a metaheuristic approach that integrates a set cover problem with an adaptive large neighborhood search (ALNS). Our ALNS approach generates a set of promising routes and micro-depot locations using destroy and repair operators while using a local search for intensification. We then utilize the set cover problem to find better network configurations. Additionally, we present a decomposition-based cluster-first, route-second approach to solve large-scale instances efficiently. We show the efficacy of our algorithm on well-known benchmark datasets and provide managerial insights based on a case study for the city of Munich. Our decomposition approach provides comparable results while reducing computational times by a factor of 15. Our case study results show that allowing direct shipment can reduce total costs by 4.7% and emissions by 11%, while increasing truck utilizations by 42%. We find that integrating both stationary and mobile micro-depots, along with allowing direct shipments, can reduce total costs by 5.9% compared to traditional two-echelon delivery structures.

==> resources/preamble.tex <==
% \documentclass[%
%     fontsize=11pt,
%     twoside=off,
%     bibliography=totoc % add references to table of content
% ]{scrartcl} % document-class: KOMA-Script Book
% \usepackage{scrlayer-scrpage}
% \usepackage[utf8]{inputenc}
% \usepackage[T1]{fontenc}
% \usepackage[english]{babel}

% % Pseudo code
% \usepackage[ruled, noend, linesnumbered]{algorithm2e}
% \SetKw{Continue}{continue}
% % \usepackage{floatrow}

% % Layout
% \usepackage[scaled]{helvet}% Helvetica as font
% \renewcommand{\familydefault}{\sfdefault}
% \usepackage[onehalfspacing]{setspace} % 1.5 spacing
% \usepackage{relsize}
% \usepackage[absolute]{textpos}
% \usepackage{tabto} % tabs

% % Figures
% \usepackage{graphicx}
% \usepackage{caption}
% \usepackage{subcaption}
% \usepackage{etoolbox}
% \usepackage{placeins}
% \usepackage{float}
% \graphicspath{{Figures/}}
% \usepackage{wrapfig}

% \usepackage{standalone}


% % Numbering
% %\usepackage{chngcntr}
% %\counterwithout{figure}{chapter}
% %\counterwithout{table}{chapter}
% %\counterwithout{footnote}{chapter}
% %\counterwithout{equation}{chapter}

% % Tables
% \usepackage{longtable}
% \usepackage{threeparttable}
% \usepackage{booktabs}
% \usepackage{array}
% \usepackage{multirow}
% \usepackage{tabularx}
% \usepackage{makecell}
% \usepackage{pdflscape}

% % Math
% \usepackage{amsmath, amsthm, amssymb, amsfonts}
% \usepackage{calc}
% \usepackage{accents}
% \newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
% \usepackage{bbm}

% % Bibliography
% \usepackage{natbib}
% \apptocmd{\thebibliography}{\raggedright}{}{}% prevent underfull hbox

% %\bibpunct[, ]{(}{)}{,}{a}{}{,} % Use INFORMS style
% %\def\bibfont{\small}
% %\def\bibsep{\smallskipamount}
% %\def\bibhang{24pt}
% %\def\newblock{\ }
% %\def\BIBand{and}
% \bibliographystyle{./resources/informs2014}

% % Natbib setup for author-year style
% \usepackage{natbib}
%  \bibpunct[, ]{(}{)}{,}{a}{}{,}%
%  \def\bibfont{\small}%
%  \def\bibsep{\smallskipamount}%
%  \def\bibhang{24pt}%
%  \def\newblock{\ }%
%  \def\BIBand{and}%
 
 
% % Abstract
% %\newenvironment{abstract}{%
% %  \titlepage%
% %  \null\vfil%
% %  \begin{center}\normalfont\usekomafont{disposition}Abstract\end{center}%
% %}{%
% %  \par%
% %  \vfil\null%
% %  \endtitlepage%
% %}

% % Misc
% \usepackage{pdfpages}
% \usepackage[hidelinks]{hyperref}
% \usepackage{enumitem}
% \usepackage{eurosym}
% \usepackage[super]{nth}
% \usepackage{lipsum}

% % Glossaries
% \usepackage[acronym,nopostdot]{glossaries}

% % TikZ
% \usepackage{tikz}
% \usetikzlibrary{calc}
% \usetikzlibrary{positioning}
% \usetikzlibrary{patterns}
% \usetikzlibrary{matrix}
% \usetikzlibrary{external}
% \usetikzlibrary{arrows}
% \usetikzlibrary{shapes}
% \usepackage{pgfplots,color}
% \usepackage{import}
% \pgfplotsset{compat=1.8}


% % Write LPs
% \usepackage{optidef}

% % Debugging:
% \usepackage{scrhack}
% %\usepackage{showframe} % Layout-Boxen anzeigen
% %\usepackage{layout} % Layout-Informationen
% %\usepackage{printlen} % Längenwerte ausgeben

% % Theorems, Definitions, etc
% \theoremstyle{definition}
% \newtheorem{definition}{Definition}[section]
% \newtheorem{theorem}{Theorem}

% % bold font
% \usepackage{bm}



